Crossing the Linguistic Causeway: A Binational Approach for Translating Soundscape Attributes to Bahasa Melayu

Translation of perceptual descriptors such as the perceived affective quality attributes in the soundscape standard (ISO/TS 12913-2:2018) is an inherently intricate task, especially if the target language is used in multiple countries. Despite geographical proximity and a shared language of Bahasa Melayu (Standard Malay), differences in culture and language education policies between Singapore and Malaysia could invoke peculiarities in the affective appraisal of sounds. To generate provisional translations of the eight perceived affective attributes -- eventful, vibrant, pleasant, calm, uneventful, monotonous, annoying, and chaotic -- into Bahasa Melayu that is applicable in both Singapore and Malaysia, a binational expert-led approach supplemented by a quantitative evaluation framework was adopted. A set of preliminary translation candidates were developed via a four-stage process, firstly by a qualified translator, which was then vetted by linguistics experts, followed by examination via an experiential evaluation, and finally reviewed by the core research team. A total of 66 participants were then recruited cross-nationally to quantitatively evaluate the preliminary translation candidates. Of the eight attributes, cross-national differences were observed only in the translation of annoying. For instance, "menjengkelkan" was found to be significantly less understood in Singapore than in Malaysia, as well as less understandable than "membingitkan" within Singapore. Results of the quantitative evaluation also revealed the imperfect nature of foreign language translations for perceptual descriptors, which suggests a possibility for exploring corrective measures.

==> sections/z05discussion.tex <==
% Discussion section
\section{Discussion}\label{sec:discussion}

\subsection{Cross-national effects on main axis attributes}
Since no statistically significant differences were found between \textsc{sg} and \textsc{my} across all evaluation criteria for \textit{pleasant} and \textit{uneventful}, the proposed translations \textit{menyenangkan} and \textit{tidak meriah} are generally applicable across both countries and agrees with the preliminary translations. Interestingly, \textit{menyenangkan} was also independently verified as the most suitable translation for \textit{pleasant} in Bahasa Indonesia (ISO 639-3: \textsc{ind}) \citep{Sudarsono2022TheStudy}. Even though \textit{meriah} (as a translation of \textit{eventful}) was significantly less understood in \textsc{sg} than \textsc{my}, albeit with weak significance and small effect size, the understandability of \textit{meriah} is still significantly high in the \textsc{sg} population ($\mu^{\textsc{sg:}\textit{meriah}}_{\textsc{undr}}=0.9$). Moreover, the \textit{meriah--tidak meriah} translation pair forms a parallelism with the \textit{eventful--uneventful} pair and should thus be used as such. Hence, \textit{menyenangkan}, \textit{meriah}, and \textit{tidak meriah} are confirmed as translations of \textit{pleasant}, \textit{eventful}, and \textit{uneventful}, respectively.

Between \textsc{sg} and \textsc{my} populations, translations for \textit{annoying} were significantly different in \textsc{undr} and \textsc{ibal} scores. As a result of a stronger implied meaning towards \textit{chaotic}, \textit{membingitkan} as a translation of \textit{annoying} in the \textsc{sg} population had significantly less implicative balance than \textit{menjengkelkan} in the \textit{my} population. However, \textit{menjengkelkan} was significantly less understandable to the layman in \textsc{sg} than in \textsc{my}. Since 95\% of the Malay-speaking population in \textsc{sg} expressed high levels of  proficiency in Bahasa Melayu \citep{Mathews2020LanguageLanguage}, the lower understandability of \textit{menjengkelkan} could be attributed to its lack of conversational use in \textsc{sg}. Basing on understandability, \textit{membingitkan} appears to be more suitable across both \textsc{sg} and \textsc{my}. Additionally, \textsc{sg:}\textit{membingitkan} and \textsc{my:}\textit{membingitkan} are similar across all evaluation criteria, and is thus suitable as a provisional translation of \textit{annoying} across \textsc{sg} and \textsc{my}. However, \textit{membingitkan} could be coupled with \textit{menjengkelkan} and should also be included when used in \textsc{my}.

\subsection{Cross-national effects on derived axis attributes}

Between countries, \textit{bersemarak} as a translation of \textit{vibrant} was significantly less understandable to a lay person in \textsc{sg} as opposed to \textit{rancak} in \textsc{my}. This lower understandability could also be attributed to \textit{bersemarak} being more uncommon in \textsc{sg}. Since \textit{rancak} was observed to be similar across both countries for all evaluation criteria, it is suitable as a provisional translation for \textit{vibrant} across \textsc{sg} and \textsc{my}.

The quantitative evaluation results of \textit{tenang} as a translation of \textit{calm} is also in agreement with the preliminary translations. Besides being binationally more appropriate than \textit{menenangkan} to a significant extent, \textit{tenang} was also more understandable in \textsc{sg} as compared to \textit{menenangkan} in \textsc{my}. Since there is a lack of evidence to suggest that there is a cross-cultural difference in \textit{tenang} (i.e., \textsc{sg:}\textit{tenang} v. \textsc{my:}\textit{tenang}), it is thus confirmed as the final provisional translation of \textit{calm}.

No significant bi-cultural differences were found within each of the three candidates for \textit{monotonous} across all evaluation criteria. All three candidates for \textit{monotonous} only differed significantly across candidates and cultures in understandability. In particular, \textit{membosankan} as a single word was significantly more understandable than its phrasal form \textit{tidak berubah oleh itu membosankan} in both \textsc{sg}-\textsc{my} and \textsc{my}-\textsc{sg} comparisons. Moreover, another phrasal variant, \textsc{sg:}\textit{kurang kepelbagaian oleh itu membosankan}, was significantly less understandable than \textsc{my:}\textit{membosankan}. Hence, \textit{membosankan} appears to be a suitable and sufficient translation for \textit{monotonous} across both countries. 

Within each of the two candidates, no significant differences were observed across \textsc{sg} and \textsc{my}. Although across candidates, \textit{huru-hara} has significantly lower clarity in \textsc{sg} than both \textit{kelam-kabut} and \textit{huru-hara} in \textsc{my}, its connotativeness was found to be significantly higher in \textsc{sg} than both candidates in \textsc{my}. This shows that \textit{huru-hara} has greater implied meanings to \textit{annoying} and \textit{eventful} in \textsc{sg}, whereas both candidates tends towards being non-connotative in \textsc{my}. Moreover, the appropriateness of \textit{huru-hara} was found to be significantly higher in \textsc{my} than \textit{kelam-kabut} in \textsc{sg}. Hence, \textit{huru-hura} appears to be suitable as a provisional translation of \textit{vibrant} across countries.

\subsection{Intra-country differences}

As a final step, a KWT was conducted to determine if intra-country differences produced any contradictory results for translations with multiple candidates (i.e., \textit{annoying, vibrant, calm, monotonous, chaotic}).

For the translation of \textit{annoying}, \textsc{sg:}\textit{membingitkan} was significantly more understandable ($p<0.01$, $0.06<\eta^2<0.14$), but had a significantly lower \textsc{ibal} score ($p<0.01$, $0.06<\eta^2<0.14$) than \textsc{sg:}\textit{menjengkelkan}. On the contrary, \textsc{my:}\textit{menjengkelkan} was both significantly more appropriate ($p<0.05$, $0.06<\eta^2<0.14$) and had higher non-connotativeness than \textsc{my:}\textit{membingitkan}. Hence, the intra-country differences suggest that both candidates should be used in conjunction, especially if used in \textsc{my}.

Intra-country differences in the translation of \textit{vibrant} was only observed within \textsc{my}, whereby \textit{rancak} was found to be more understandable than \textit{bersemarak}. Therefore, a singular translation via \textit{rancak} was deemed sufficient.

For the translation of \textit{calm}, \textsc{sg:}\textit{tenang} was found to be significantly more appropriate ($p<0.001$, $\eta^2>0.14$) and understandable ($p<0.001$, $\eta^2>0.14$) than \textsc{sg:}\textit{menenangkan}. Similarly, \textsc{my:}\textit{tenang} was significantly more appropriate ($p<0.001$,  $\eta^2>0.14$) and understandable ($p<0.05$, $0.06<\eta^2<0.14$) than \textsc{my:}\textit{menenangkan}. Thus, the singular translation in \textit{tenang} is consistent with the bi-cultural analysis.

Across the three candidates for \textit{monotonous}, significant differences were found only in \textsc{undr} in \textsc{sg} ($p<0.01$, $0.06<\eta^2<0.14$), but in both \textsc{appr} ($p<0.05$, $0.06<\eta^2<0.14$) and \textsc{undr} ($p<0.001$, $\eta^2>0.14$) in \textsc{my} in the KWTs. Post-hoc CIT revealed that \textsc{sg:}\textit{membosankan} was significantly more understandable than both its phrasal variants \textsc{sg:}\textit{tidak berubah oleh itu membosankan} ($p<0.01$) and \textsc{sg:}\textit{kurang kepelbagaian oleh itu membosankan} ($p<0.01$). Likewise,  \textsc{my:}\textit{membosankan} was significantly more understandable than \textsc{my:}\textit{tidak berubah oleh itu membosankan} ($p<0.001$) and \textsc{my:}\textit{kurang kepelbagaian oleh itu membosankan} ($p<0.05$). Although \textsc{my:}\textit{kurang kepelbagaian oleh itu membosankan} had significantly higher appropriateness over \textsc{my:}\textit{tidak berubah oleh itu membosankan} ($p<0.05$), it was similarly appropriate to \textsc{my:}\textit{membosankan}. In line with the bi-cultural analysis, the singular \textit{membosankan} is thus the most suitable translation for \textit{monotonous}.

Lastly, significant differences were observed only in \textsc{appr} within both \textsc{sg} ($p<0.001$, $\eta^2>0.14$) and \textsc{my} ($p<0.01$,$0.06<\eta^2<0.14$) for the translation of \textit{chaotic}. Since \textit{huru-hara} in both \textsc{sg} and \textsc{my} was significantly more appropriate than \textit{kelam-kabut} in each country respectively, this provides further evidence that \textit{huru-hara} is suitable across and within countries as a translation of \textit{chaotic}.

\input{table/finaltrans}

\subsection{Final provisional translations of PAQ attributes to ISO 639-3: \textsc{zsm}}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.45\linewidth]{fig/mainRadar_0.4-1.0.png}
    \includegraphics[width=0.45\linewidth]{fig/derivedRadar_0.4-1.0.png}
    \caption{Mean scores of all participants across all criteria in stage 1e for the provisional translations of main axis (left) and derived axis (right) attributes}
    \label{fig:radarFinaltrans}
\end{figure*}

Based on the inter- and intra-country analysis of stage 1e, the final set of provisional translations for ISO 639-3:\textsc{zsm} are summarised in \Cref{tab:provtrans}. Except for \textit{annoying}, all other attributes are represented by a single-word translation in \textsc{zsm} that are viable across both Singapore and Malaysia. For \textit{annoying}, \textit{membingitkan} was selected for \textsc{sg} based on its significantly greater understandability, whereas both \textit{membingitkan} in conjuction with \textit{menjengkelkan} were suggested for \textsc{my}. The binational difference in the provisional translation of \textit{annoying} warrants further investigation and verification in the form of listening tests.

Visualisation of the mean criteria scores of the main axis and derived axis attribute translations in (\Cref{fig:radarFinaltrans}), also reveals potential non-compliance with the assumed circumplexity of the perceived affective quality model in ISO 12913-3. It should be noted that the low \textsc{anto}, \textsc{orth}, \textsc{ncon}, and \textsc{ibal} scores directly affect the integrity of the main axis assumptions, for example in \textit{meriah}. Likewise, low \textsc{conn} and \textsc{ibal} scores also affect the structural integrity of the derived axes, for instance in \textit{membosankan}. Hence, there is an impetus to further investigate the circumplexity of the \textsc{zsm} translations as well as means for calibration or compensation for the equations in ISO 12913-3 to be valid. 





==> unused/04quant.tex <==
% Quantitative evaluation section

\section{Stage 1e: quantitative evaluation}\label{sec:quant}


Since the differences between Singapore and Malaysia respondents are being investigated, 3 (\SI{4.55}{\percent}) of the 66 participants whose self-reported current countries of residence (CCR) are outside of Singapore (\textsc{sg}) and Malaysia (\textsc{my}) were excluded in the analyses. Where more than one translation candidate per PAQ attribute were assessed, the differences were evaluated via Kruskal-Wallis tests \citep[KWT;][]{Kruskal1952UseAnalysis} while considering all the respondents either as a single population (``combined'') or split across their self-reported CCR (``split''). Only if a statistically significant difference in distributions were found, a post-hoc Conover-Iman test \citep[CIT;][]{Conover1979OnProcedures} was employed to investigate the pairwise differences in both the combined and split cases when there are more than one pair of candidates assessed. For cases where only one candidate was assessed, only the differences across the CCR split (i.e., \textsc{my} v. \textsc{sg}) could be evaluated. The mean scores of both the combined and split cases for the main and derived axis candidates are summarised in \cref{tab:main_scores} and \cref{tab:derived_scores}, respectively. Additionally, the $p$-values of the KWT and CIT analyses are summarised in \Cref{tab:citp}.

\subsection{Main axes} 

Based on the preliminary translations in Stage 1d, only one translation candidate was selected for \textit{eventful}, \textit{pleasant}, and \textit{uneventful}, i.e., \imeriah{}, \imenye{}, and \itimer{}, respectively, whereas there were two candidates to be evaluated for \textit{annoying} -- \membi{} and \menje{}. The main axis translation candidates were evaluated on their \textsc{appr}, \textsc{undr}, \textsc{clar}, \textsc{anto}, \textsc{orth}, \textsc{ncon}, and \textsc{ibal}

\subsubsection{Single translation candidate (\textit{eventful}, \textit{pleasant} and \textit{uneventful})}

Although inter-candidate comparison for attribute with a single translation can not be made, the applicability of these candidates were thus evaluated across the CCR via the KWT. No significant differences were found between \textsc{my} and \textsc{sg} for all evaluation criteria (\textsc{appr}, \textsc{undr}, \textsc{clar}, \textsc{anto}, \textsc{orth}, \textsc{ncon}, \textsc{ibal}) on translations of \textit{pleasant} and \textit{uneventful} (i.e., \imenye{}, and \itimer{}, respectively). For the translation of \textit{eventful} (i.e., \imeriah{}), no significant differences were found across all criteria with the exception of \textsc{undr} ($p<0.05$), albeit with weak significance. Hence, translations of \textit{eventful}, \textit{pleasant}, and \textit{uneventful} appear to be suitable across \textsc{my} and \textsc{sg}.

\subsubsection{Multiple  translation candidates (\textit{annoying})}

The differences between the two translation candidates for \textit{annoying} --- \imembi{} and \imenje{} --- were evaluated via KWT on all criteria in the combined population. Significant differences were found for \textsc{undr} ($p<0.01$; $\eta^2<0.06$), \textsc{ncon} ($p<0.05$; $\eta^2<0.06$), and \textsc{ibal} ($p<0.001$; $0.06<\eta^2<0.14$). Although \imembi{} ($\mu_{\textsc{undr}}=0.773$) is more easily understood than \imenje{} ($\mu_{\textsc{undr}}=0.711$), \imenje{} ($\mu_{\textsc{ncon}}=0.649, \mu_{\textsc{ibal}}=0.756$) appears to have significantly greater non-connotativeness and implicative balance than \imembi{} ($\mu_{\textsc{ncon}}=0.554$, $\mu_{\textsc{ibal}}=0.565$), as shown in \Cref{tab:main_scores}. Whereas differences in \textsc{ibal} had a moderate effect, only a small effect was observed for \textsc{undr} and \textsc{ncon}. 

Unlike the KWT across candidates in the combined population, significant differences were observed in the split case with moderate effect in \textsc{undr} ($p<0.01$; $0.06<\eta^2<0.14$) and \textsc{ibal} ($p<0.01$; $0.06<\eta^2<0.14$ ), but not in \textsc{ncon}. The post-hoc CIT showed a significant differences only between \ccomp{my}{menjengkelkan}{sg}{menjengkelkan} ($p<0.01$) for \textsc{undr}. This indicates that \menje{} is significantly more understandable in \textsc{my} ($\mu^{\textit{\textsc{my:}menje}}_{\textsc{undr}}=0.823$) than in \textsc{sg} ($\mu^{\textit{\textsc{sg:}menje}}_{\textsc{undr}}=0.609$).

\subsection{Derived Axes}

The translation candidates for derived axis attributes were evaluated on their \textsc{appr}, \textsc{undr}, \textsc{clar}, \textsc{ibal} and \textsc{conn}. Two candidates were evaluated for translations of \textit{vibrant} (i.e., \irancak{}, \iberse{}), \textit{calm} (i.e., \itenang{}, \imenen{}), and \textit{chaotic} (i.e., \ihuru{}, \ikelam{}). For \textit{monotonous}, there were three candidates under evaluation (i.e., \imembo{}, \itiber{}, \ikurang{}).

\subsubsection{Vibrant}

Between candidates, significant differences were only found in \textsc{undr} in the combined case via KWT ($p<0.05$, $\eta^2<0.06$). On the whole, \irancak{} ($\mu^{\textit{ranca}}_{\textsc{undr}}=0.797$) was significantly more understandable ($p<0.01$) than \iberse{} ($\mu^{\textit{berse}}_{\textsc{undr}}=0.689$), albeit with a small effect size.  

In the split case between \textsc{my} and \textsc{sg} populations, significant differences were found also only in \textsc{undr} ($p<0.05$, $0.06<\eta^2<0.14$). However, the post-hoc CIT revealed that there were no significant differences between countries for each candidate. 

\subsubsection{Calm}

In the combined case, the translation candidates for \textit{calm} were found to be significantly different via KWT with a large effect size for both \textsc{appr} ($p<0.001$, $\eta^2>0.14$) and \textsc{undr} ($p<0.001$, $\eta^2>0.14$). Hence, \itenang{} was significantly more appropriate ($\mu^{\textit{tenan}}_{\textsc{appr}}=0.968$) and understandable ($\mu^{\textit{tenan}}_{\textsc{undr}}=0.979$) than \imenen ($\mu^{\textit{menen}}_{\textsc{appr}}=0.838$, $\mu^{\textit{menen}}_{\textsc{undr}}=0.910$).

There were also differences in the split case between \textsc{my} and \textsc{sg} populations for both \textsc{appr} ($p<0.001$, $\eta^2>0.14$) and \textsc{undr} ($p<0.001$, $\eta^2>0.14$) via KWT with a large effect size. However, the post-hoc CIT did not reveal significant differences between countries for each candidate.

\subsubsection{Monotonous}

Across the three translation candidates for \textit{monotonous}, without accounting for CCR, differences were significant only for \textsc{appr} ($p<0.05$, $\eta^2<0.06$) with a small effect size, and \textsc{undr} ($p<0.001$, 0.06<$\eta^2<0.14$) with a moderate effect size. Post-hoc CIT for \textsc{appr} showed that the differences were significant between \pcomp{membosankan}{tidak berubah oleh itu membosankan} ($p<0.05$) and \pcomp{kurang kepelbagaian oleh itu membosankan}{tidak berubah oleh itu membosankan} ($p<0.05$) pairs. Hence, \imembo{} and \ikurang{} are each significantly more appropriate than \itiber{} ($\mu^{\textit{membo}}_{\textsc{appr}}=0.765$, $\mu^{\textit{kkoim}}_{\textsc{appr}}=0.776$, $\mu^{\textit{tboim}}_{\textsc{appr}}=0.654$). In the post-hoc CIT of \textsc{undr}, differences were significant between the \pcomp{membosankan}{tidak berubah oleh itu membosankan} ($p<0.001$) and the \pcomp{membosankan}{kurang kepelbagaian oleh itu membosankan} ($p<0.001$) pairs. Hence, \imembo{} was significantly more understandable than either \itiber{} or \ikurang{} ($\mu^{\textit{membo}}_{\textsc{undr}}=0.946$, $\mu^{\textit{kkoim}}_{\textsc{undr}}=0.805$, $\mu^{\textit{tboim}}_{\textsc{undr}}=0.765$).

In the split case, the KWT showed significant differences also only for \textsc{appr} ($p<0.05$, $\eta^2<0.06$) with a small effect size, and \textsc{undr} ($p<0.001$, $0.06<\eta^2<0.14$) with a moderate effect size. In the post-hoc CIT for \textsc{appr}, there was insufficient evidence to indicate a difference in appropriateness of all attribute pairs across CCR. However, significant differences were observed in \textsc{undr} between \ccomp{sg}{membosankan}{my}{tidak berubah oleh itu membosankan} ($p<0.001$), \ccomp{my}{membosankan}{sg}{tidak berubah oleh itu membosankan} ($p<0.001$), and \ccomp{my}{membosankan}{sg}{kurang kepelbagaian oleh itu membosankan} ($p<0.05$) pairs. Therefore, \imembo{} in the context of \textsc{sg} is significantly more understandable than \itiber{} in \textsc{my}, and vice versa ($\mu^{\textit{\textsc{sg:}membo}}_{\textsc{undr}}=0.936$, $\mu^{\textit{\textsc{my:}membo}}_{\textsc{undr}}=0.957$, $\mu^{\textit{\textsc{sg:}tboim}}_{\textsc{undr}}=0.776$, $\mu^{\textit{\textsc{my:}tboim}}_{\textsc{undr}}=0.753$). Also, \imembo{} in \textsc{my} is significantly more understandable than \ikurang{} in \textsc{sg} ($\mu^{\textit{\textsc{sg:}kkoim}}_{\textsc{undr}}=0.778$).

\subsubsection{Chaotic}

Without considering the CCR, the KWT only revealed significant differences in \textsc{appr} ($p<0.001$, $\eta^2>0.14$) with a large effect size. Hence, \ihuru{} ($\mu^{\textit{huru}}_{\textsc{appr}}=0.946$) was significantly more appropriate than \textit{kelam-kabut} ($\mu^{\textit{kelam}}_{\textsc{appr}}=0.790$). Across the CCR, the KWT exhibited significant differences in \textsc{appr} ($p<0.001$, $\eta^2>0.14$), \textsc{clar} ($p<0.01$, $\eta^2<0.06$), and \textsc{conn} ($p<0.01$, $\eta^2<0.06$). 

Post-hoc CIT for \textsc{appr} showed significant differences between \ccomp{my}{huru-hara}{sg}{kelam-kabut}. The candidate \ihuru{} in the context of \textsc{my} appears to be significantly more appropriate than \textit{kelam-kabut} in \textsc{sg} ($\mu^{\textit{\textsc{my:}huru}}_{\textsc{appr}}=0.973$, $\mu^{\textit{\textsc{sg:}kelam}}_{\textsc{appr}}=0.709$).

In terms of \textsc{clar}, the CIT showed significant differences between \ccomp{my}{huru-hara}{sg}{huru-hara} ($p<0.01$) and \ccomp{my}{kelam-kabut}{sg}{huru-hara} ($p<0.05$). Hence, \ihuru{} seems to be of significantly higher clarity in \textsc{my} than \textsc{sg} ($\mu^{\textit{\textsc{my:}huru}}_{\textsc{clar}}=0.715$,$\mu^{\textit{\textsc{sg:}huru}}_{\textsc{clar}}=0.522$). Moreover, the clarity of \textit{kelam-kabut} in \textsc{my} is significantly higher than \ihuru{} in \textsc{sg}, albeit with weaker significance ($\mu^{\textit{\textsc{my:}kelam}}_{\textsc{clar}}=0.683$).

Lastly, differences in \textsc{conn} were significant in the CIT between \ccomp{sg}{huru-hara}{my}{kelam-kabut} and <\textsc{sg}{huru-hara}{my}{huru-hara} pairs. Hence, \ihuru{} has significantly higher connotativeness in \textsc{sg} than in \textsc{my} ($\mu^{\textit{\textsc{sg:}huru}}_{\textsc{conn}}=0.547$, $\mu^{\textit{\textsc{my:}huru}}_{\textsc{conn}}=0.380$), as well as over \textit{kelam-kabut} in \textsc{my} $\mu^{\textit{\textsc{my:}kelam}}_{\textsc{conn}}=0.367$. 

\input{table/main_scores}

\input{table/derived_scores}

==> unused/Rtest.tex <==
\begin{table}

\caption{Kruskal-Wallis Test on attributes with single 
  translation candidates}
\centering
\begin{tabular}[t]{rrrrr}
\toprule
Test & Attribute & Criterion & p-value & Effect size\\
\midrule
 & eventful &  & 0.5877674 & -0.0115763\\

 & pleasant &  & 0.3518312 & -0.0021829\\

 & uneventful & \multirow[t]{-3}{*}{\raggedleft\arraybackslash APPR} & 0.4094157 & -0.0052378\\
\cmidrule{2-5}
 & eventful &  & 0.0411431 & 0.0519690\\

 & pleasant &  & 0.8224231 & -0.0155677\\

 & uneventful & \multirow[t]{-3}{*}{\raggedleft\arraybackslash UNDR} & 0.1163393 & 0.0240315\\
\cmidrule{2-5}
 & eventful &  & 0.0919598 & 0.0301595\\

 & pleasant &  & 0.1782062 & 0.0133200\\

 & uneventful & \multirow[t]{-3}{*}{\raggedleft\arraybackslash CLAR} & 0.1570341 & 0.0164354\\
\cmidrule{2-5}
 & eventful &  & 0.2882946 & 0.0020913\\

 & pleasant &  & 0.0894496 & 0.0308894\\

 & uneventful & \multirow[t]{-3}{*}{\raggedleft\arraybackslash IBAL} & 0.9555434 & -0.0163425\\
\cmidrule{2-5}
 & eventful &  & 0.3825060 & -0.0038913\\

 & pleasant &  & 0.6561170 & -0.0131430\\

 & uneventful & \multirow[t]{-3}{*}{\raggedleft\arraybackslash ANTO} & 0.7023484 & -0.0139993\\
\cmidrule{2-5}
 & eventful &  & 0.1964978 & 0.0109543\\

 & pleasant &  & 0.5809662 & -0.0113988\\

 & uneventful & \multirow[t]{-3}{*}{\raggedleft\arraybackslash ORTH} & 0.6914382 & -0.0138109\\
\cmidrule{2-5}
 & eventful &  & 0.0651774 & 0.0393522\\

 & pleasant &  & 0.0511030 & 0.0459819\\

\multirow[t]{-21}{*}{\raggedleft\arraybackslash KWT} & uneventful & \multirow[t]{-3}{*}{\raggedleft\arraybackslash NCON} & 0.4988093 & -0.0088940\\
\bottomrule
\end{tabular}
\end{table}

==> unused/citpx.tex <==
\begin{sffamily}
\begin{nolinenumbers}
\small%
\noindent\textbf{\color{scolor}Table \thetable}\par%
\noindent{$p$-values of the Kruskal--Wallis tests and the posthoc Conover--Iman tests. Double asterisks (**) and single asterisk (*) indicate statistical significance at \SI{1}{\percent} and \SI{5}{\percent}, respectively. For Conover--Iman tests, the pairwise tests are listed in the order of increasing $p$-value, and the candidate translation with the higher average score in the respective criterion is always listed on the left of each pair.}%
% \par\vskip12pt
\end{nolinenumbers}
\small%
\begin{longtable}{lll@{\hskip3pt}>{\raggedright}p{4cm}cl@{\hskip3pt}>{\raggedright}p{4cm}rl}
% first head
    \toprule
    Eng. Attr. &
    Criterion &
    \multicolumn{5}{l}{Statistical Test} &
    $p$-value\\
    % \midrule
\endfirsthead

% head
    \toprule
    Eng. Attr. &
    Criteria &
    \multicolumn{5}{l}{Statistical Test} &
    $p$-value\\
    \midrule
\endhead

    % \cmidrule{7-9}
    \\
    \multicolumn{9}{r}{[Continued on next page]} \\
    % \midrule
\endfoot

    \bottomrule
    \label{tab:citp}
\endlastfoot

\midrule Pleasant & APPR & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.352 & \\*
\cmidrule{2-9}
 & UNDR & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.822 & \\*
\cmidrule{2-9}
 & CLAR & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.370 & \\*
\cmidrule{2-9}
 & ANTO & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.656 & \\*
\cmidrule{2-9}
 & ORTH & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.601 & \\*
\cmidrule{2-9}
 & NCON & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.200 & \\*
\cmidrule{2-9}
 & IBAL & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.087 & \\
\midrule Annoying & APPR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.073 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.073 & \\*
\cmidrule{2-9}
 & UNDR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.163 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.008 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (split)} & & \\*
 & & MY & menjengkelkan & v & SG & menjengkelkan & 0.008 & ** \\*
 & & SG & membingitkan & v & SG & menjengkelkan & 0.041 & * \\*
 & & MY & membingitkan & v & SG & menjengkelkan & 0.089 & \\*
 & & MY & menjengkelkan & v & MY & membingitkan & $\approx$1.000 & \\*
 & & SG & membingitkan & v & MY & membingitkan & $\approx$1.000 & \\*
 & & MY & menjengkelkan & v & SG & membingitkan & $\approx$1.000 & \\*
\cmidrule{2-9}
 & CLAR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.384 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.560 & \\*
\cmidrule{2-9}
 & ANTO & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.650 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.695 & \\*
\cmidrule{2-9}
 & ORTH & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.334 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.446 & \\*
\cmidrule{2-9}
 & NCON & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.025 & * \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (combined)} & & \\*
 & &  & menjengkelkan & v &  & membingitkan & 0.025 & * \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.100 & \\*
\cmidrule{2-9}
 & IBAL & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (combined)} & & \\*
 & &  & menjengkelkan & v &  & membingitkan & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.003 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (split)} & & \\*
 & & MY & menjengkelkan & v & SG & membingitkan & 0.003 & ** \\*
 & & SG & menjengkelkan & v & SG & membingitkan & 0.014 & * \\*
 & & MY & membingitkan & v & SG & membingitkan & 0.440 & \\*
 & & MY & menjengkelkan & v & MY & membingitkan & 0.476 & \\*
 & & SG & menjengkelkan & v & MY & membingitkan & $\approx$1.000 & \\*
 & & MY & menjengkelkan & v & SG & menjengkelkan & $\approx$1.000 & \\
\midrule Eventful & APPR & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.588 & \\*
\cmidrule{2-9}
 & UNDR & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.041 & * \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (split)} & & \\*
 & & MY & meriah & v & SG & meriah & 0.040 & * \\*
\cmidrule{2-9}
 & CLAR & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.203 & \\*
\cmidrule{2-9}
 & ANTO & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.383 & \\*
\cmidrule{2-9}
 & ORTH & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.236 & \\*
\cmidrule{2-9}
 & NCON & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.184 & \\*
\cmidrule{2-9}
 & IBAL & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.352 & \\
\midrule Uneventful & APPR & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.409 & \\*
\cmidrule{2-9}
 & UNDR & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.116 & \\*
\cmidrule{2-9}
 & CLAR & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.078 & \\*
\cmidrule{2-9}
 & ANTO & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.702 & \\*
\cmidrule{2-9}
 & ORTH & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.712 & \\*
\cmidrule{2-9}
 & NCON & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.495 & \\*
\cmidrule{2-9}
 & IBAL & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.994 & \\
\midrule Calm & APPR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (combined)} & & \\*
 & &  & tenang & v &  & menenangkan & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (split)} & & \\*
 & & SG & tenang & v & MY & menenangkan & <0.001 & ** \\*
 & & SG & tenang & v & SG & menenangkan & <0.001 & ** \\*
 & & MY & tenang & v & MY & menenangkan & 0.002 & ** \\*
 & & MY & tenang & v & SG & menenangkan & 0.038 & * \\*
 & & SG & menenangkan & v & MY & menenangkan & $\approx$1.000 & \\*
 & & SG & tenang & v & MY & tenang & $\approx$1.000 & \\*
\cmidrule{2-9}
 & UNDR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (combined)} & & \\*
 & &  & tenang & v &  & menenangkan & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (split)} & & \\*
 & & SG & tenang & v & MY & menenangkan & <0.001 & ** \\*
 & & SG & tenang & v & SG & menenangkan & 0.001 & ** \\*
 & & MY & tenang & v & MY & menenangkan & 0.037 & * \\*
 & & MY & tenang & v & SG & menenangkan & 0.098 & \\*
 & & MY & menenangkan & v & SG & menenangkan & $\approx$1.000 & \\*
 & & SG & tenang & v & MY & tenang & $\approx$1.000 & \\*
\cmidrule{2-9}
 & CLAR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.447 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.439 & \\*
\cmidrule{2-9}
 & CONN & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.507 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.405 & \\*
\cmidrule{2-9}
 & IBAL & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.941 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.792 & \\
\midrule Chaotic & APPR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (combined)} & & \\*
 & &  & huru-hara & v &  & kelam-kabut & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (split)} & & \\*
 & & MY & huru-hara & v & SG & kelam-kabut & <0.001 & ** \\*
 & & SG & huru-hara & v & SG & kelam-kabut & <0.001 & ** \\*
 & & MY & huru-hara & v & MY & kelam-kabut & 0.062 & \\*
 & & MY & kelam-kabut & v & SG & kelam-kabut & 0.076 & \\*
 & & SG & huru-hara & v & MY & kelam-kabut & 0.898 & \\*
 & & MY & huru-hara & v & SG & huru-hara & $\approx$1.000 & \\*
\cmidrule{2-9}
 & UNDR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.847 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.545 & \\*
\cmidrule{2-9}
 & CLAR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.299 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.002 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (split)} & & \\*
 & & MY & huru-hara & v & SG & huru-hara & 0.002 & ** \\*
 & & MY & kelam-kabut & v & SG & huru-hara & 0.011 & * \\*
 & & SG & kelam-kabut & v & SG & huru-hara & 0.290 & \\*
 & & MY & huru-hara & v & SG & kelam-kabut & 0.483 & \\*
 & & MY & huru-hara & v & MY & kelam-kabut & $\approx$1.000 & \\*
 & & MY & kelam-kabut & v & SG & kelam-kabut & $\approx$1.000 & \\*
\cmidrule{2-9}
 & CONN & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.225 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.006 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (split)} & & \\*
 & & SG & huru-hara & v & MY & kelam-kabut & 0.012 & * \\*
 & & SG & huru-hara & v & MY & huru-hara & 0.019 & * \\*
 & & SG & kelam-kabut & v & MY & kelam-kabut & 0.661 & \\*
 & & SG & huru-hara & v & SG & kelam-kabut & 0.711 & \\*
 & & SG & kelam-kabut & v & MY & huru-hara & 0.890 & \\*
 & & MY & huru-hara & v & MY & kelam-kabut & $\approx$1.000 & \\*
\cmidrule{2-9}
 & IBAL & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.933 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.640 & \\
\midrule Vibrant & APPR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.241 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.413 & \\*
\cmidrule{2-9}
 & UNDR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.010 & * \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (combined)} & & \\*
 & &  & rancak & v &  & bersemarak & 0.010 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.013 & * \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (split)} & & \\*
 & & MY & rancak & v & SG & bersemarak & 0.007 & ** \\*
 & & MY & rancak & v & MY & bersemarak & 0.177 & \\*
 & & MY & rancak & v & SG & rancak & 0.441 & \\*
 & & SG & rancak & v & SG & bersemarak & 0.717 & \\*
 & & MY & bersemarak & v & SG & bersemarak & $\approx$1.000 & \\*
 & & SG & rancak & v & MY & bersemarak & $\approx$1.000 & \\*
\cmidrule{2-9}
 & CLAR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.601 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.110 & \\*
\cmidrule{2-9}
 & CONN & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.639 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.261 & \\*
\cmidrule{2-9}
 & IBAL & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.587 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.811 & \\
\midrule Monotonous & APPR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.012 & * \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (combined)} & & \\*
 & &  & membosankan & v &  & tidak berubah oleh itu membosankan & 0.019 & * \\*
 & &  & kurang kepelbagaian oleh itu membosankan & v &  & tidak berubah oleh itu membosankan & 0.044 & * \\*
 & &  & kurang kepelbagaian oleh itu membosankan & v &  & membosankan & $\approx$1.000 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.041 & * \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (split)} & & \\*
 & & SG & membosankan & v & MY & tidak berubah oleh itu membosankan & 0.061 & \\*
 & & MY & kurang kepelbagaian oleh itu membosankan & v & MY & tidak berubah oleh itu membosankan & 0.080 & \\*
 & & MY & membosankan & v & MY & tidak berubah oleh itu membosankan & 0.252 & \\*
 & & SG & kurang kepelbagaian oleh itu membosankan & v & MY & tidak berubah oleh itu membosankan & 0.521 & \\*
 & & MY & kurang kepelbagaian oleh itu membosankan & v & MY & membosankan & $\approx$1.000 & \\*
 & & MY & kurang kepelbagaian oleh itu membosankan & v & SG & kurang kepelbagaian oleh itu membosankan & $\approx$1.000 & \\*
 & & MY & kurang kepelbagaian oleh itu membosankan & v & SG & membosankan & $\approx$1.000 & \\*
 & & MY & kurang kepelbagaian oleh itu membosankan & v & SG & tidak berubah oleh itu membosankan & $\approx$1.000 & \\*
 & & SG & kurang kepelbagaian oleh itu membosankan & v & MY & membosankan & $\approx$1.000 & \\*
 & & SG & membosankan & v & MY & membosankan & $\approx$1.000 & \\*
 & & MY & membosankan & v & SG & tidak berubah oleh itu membosankan & $\approx$1.000 & \\*
 & & SG & tidak berubah oleh itu membosankan & v & MY & tidak berubah oleh itu membosankan & $\approx$1.000 & \\*
 & & SG & membosankan & v & SG & kurang kepelbagaian oleh itu membosankan & $\approx$1.000 & \\*
 & & SG & kurang kepelbagaian oleh itu membosankan & v & SG & tidak berubah oleh itu membosankan & $\approx$1.000 & \\*
 & & SG & membosankan & v & SG & tidak berubah oleh itu membosankan & $\approx$1.000 & \\*
\cmidrule{2-9}
 & UNDR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (combined)} & & \\*
 & &  & membosankan & v &  & tidak berubah oleh itu membosankan & <0.001 & ** \\*
 & &  & membosankan & v &  & kurang kepelbagaian oleh itu membosankan & <0.001 & ** \\*
 & &  & kurang kepelbagaian oleh itu membosankan & v &  & tidak berubah oleh itu membosankan & 0.541 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & <0.001 & ** \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Conover-Iman (split)} & & \\*
 & & MY & membosankan & v & MY & tidak berubah oleh itu membosankan & <0.001 & ** \\*
 & & SG & membosankan & v & MY & tidak berubah oleh itu membosankan & <0.001 & ** \\*
 & & MY & membosankan & v & SG & tidak berubah oleh itu membosankan & 0.009 & ** \\*
 & & SG & membosankan & v & SG & tidak berubah oleh itu membosankan & 0.012 & * \\*
 & & MY & membosankan & v & SG & kurang kepelbagaian oleh itu membosankan & 0.023 & * \\*
 & & SG & membosankan & v & SG & kurang kepelbagaian oleh itu membosankan & 0.032 & * \\*
 & & MY & membosankan & v & MY & kurang kepelbagaian oleh itu membosankan & 0.142 & \\*
 & & SG & membosankan & v & MY & kurang kepelbagaian oleh itu membosankan & 0.193 & \\*
 & & MY & kurang kepelbagaian oleh itu membosankan & v & MY & tidak berubah oleh itu membosankan & $\approx$1.000 & \\*
 & & MY & kurang kepelbagaian oleh itu membosankan & v & SG & kurang kepelbagaian oleh itu membosankan & $\approx$1.000 & \\*
 & & MY & kurang kepelbagaian oleh itu membosankan & v & SG & tidak berubah oleh itu membosankan & $\approx$1.000 & \\*
 & & MY & membosankan & v & SG & membosankan & $\approx$1.000 & \\*
 & & SG & kurang kepelbagaian oleh itu membosankan & v & MY & tidak berubah oleh itu membosankan & $\approx$1.000 & \\*
 & & SG & tidak berubah oleh itu membosankan & v & MY & tidak berubah oleh itu membosankan & $\approx$1.000 & \\*
 & & SG & kurang kepelbagaian oleh itu membosankan & v & SG & tidak berubah oleh itu membosankan & $\approx$1.000 & \\*
\cmidrule{2-9}
 & CLAR & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.847 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.929 & \\*
\cmidrule{2-9}
 & CONN & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.600 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.874 & \\*
\cmidrule{2-9}
 & IBAL & \multicolumn{5}{l}{Kruskal-Wallis (combined)} & 0.882 & \\
\cmidrule{3-9}
 & & \multicolumn{5}{l}{Kruskal-Wallis (split)} & 0.400 & \\
\end{longtable}
\end{sffamily}

==> unused/derived_scores.tex <==

\begin{landscape}
\begin{table}[t]
    \caption{Evaluation scores for attributes on the derived axes. Double asterisks (**) and single asterisk (*) with boldface indicate that the distribution underlying the score is significantly different from those of \textbf{all} other candidates, at \SI{1}{\percent} and \SI{5}{\percent} significance levels using the pairwise posthoc Conover-Iman test with Bonferroni corrections, respectively. For candidates with at least one but not all statistically significant posthoc tests, the oplus ($^{\oplus}$) sign indicates the number of pairwise tests where the null hypotheses are rejected at \SI{1}{\percent} significance level. The plus ($^{+}$) sign indicates the number of pairwise tests where the null hypotheses are rejected at \SI{5}{\percent} significance level but not at \SI{1}{\percent}.}
    % \tiny
    \setlength{\tabcolsep}{3pt}
    \label{tab:derived_scores}
    \renewcommand*{\arraystretch}{1.1}
    \centering
    \begin{tabularx}{\linewidth}{%
        l>{\raggedright\arraybackslash}p{3.1cm}
        *{15}{>{\raggedleft\arraybackslash}X}}
    \toprule
    Eng. Attr. &
    Trans. &
    \multicolumn{3}{c}{\uppercase{appr}} &
    \multicolumn{3}{c}{\uppercase{undr}} &
    \multicolumn{3}{c}{\uppercase{clar}} &
    \multicolumn{3}{c}{\uppercase{conn}} &
    \multicolumn{3}{c}{\uppercase{ibal}} \\
    \cmidrule(lr){3-5}
    \cmidrule(lr){6-8}
    \cmidrule(lr){9-11}
    \cmidrule(lr){12-14}
    \cmidrule(lr){15-17}
    && 
    Com & MY & SG &
    Com & MY & SG &
    Com & MY & SG &
    Com & MY & SG &
    Com & MY & SG \\
    \midrule
    calm & menenangkan &             0.838 &            0.817 &             0.858 &             0.910 &             0.910 &            0.909 &  0.482 &  0.528 &  0.439 &  0.589 &  0.537 &  0.636 &  0.584 &  0.533 &  0.630 \\
        & tenang &  **\textbf{0.968} &  *\textbf{0.953} &  **\textbf{0.982} &  **\textbf{0.979} &   *\textbf{0.963} &  *\textbf{0.994} &  0.514 &  0.510 &  0.518 &  0.613 &  0.597 &  0.629 &  0.586 &  0.580 &  0.591 \\\midrule
chaotic & huru-hara &  **\textbf{0.946} &            0.973 &  **\textbf{0.921} &             0.954 &             0.967 &            0.942 &  0.614 &  0.715 &  0.523 &  0.467 &  0.380 &  0.547 &  0.713 &  0.747 &  0.682 \\
        & kelam-kabut &             0.790 &            0.880 &             0.709 &             0.948 &             0.970 &            0.927 &  0.655 &  0.683 &  0.629 &  0.414 &  0.367 &  0.458 &  0.708 &  0.733 &  0.685 \\ \midrule
monotonous 
        & membosankan &       $^{+}$0.765 &            0.750 &             0.779 &  **\textbf{0.946} &  $^{\oplus}$0.957 &  *\textbf{0.936} &  0.549 &  0.578 &  0.523 &  0.496 &  0.493 &  0.498 &  0.529 &  0.540 &  0.518 \\
        & tidak berubah oleh itu membosankan &             0.654 &            0.617 &             0.688 &             0.765 &             0.753 &            0.776 &  0.564 &  0.573 &  0.556 &  0.454 &  0.438 &  0.468 &  0.546 &  0.597 &  0.500 \\
        & kurang kepelbagaian oleh itu membosankan &       $^{+}$0.776 &            0.787 &             0.767 &             0.805 &             0.833 &            0.779 &  0.537 &  0.543 &  0.530 &  0.486 &  0.462 &  0.508 &  0.562 &  0.643 &  0.488 \\\midrule
vibrant & bersemarak &             0.790 &            0.743 &             0.833 &             0.689 &             0.737 &            0.645 &  0.456 &  0.508 &  0.408 &  0.623 &  0.607 &  0.638 &  0.744 &  0.760 &  0.730 \\
        & rancak &             0.722 &            0.707 &             0.736 &   *\textbf{0.797} &             0.853 &            0.745 &  0.475 &  0.507 &  0.447 &  0.607 &  0.557 &  0.653 &  0.716 &  0.680 &  0.748 \\
    \bottomrule 
    \end{tabularx}
\end{table}
\end{landscape}

==> unused/main_scores.tex <==
\newcommand{\tablegend}{Double asterisks (**) and single asterisk (*) with boldface indicate that the distribution underlying the score is significantly different from those of \textbf{all} other candidates, at \SI{1}{\percent} and \SI{5}{\percent} significance levels using the pairwise posthoc Conover-Iman test with Bonferroni corrections, respectively. 
% For candidates with at least one but not all statistically significant posthoc tests, the oplus ($^{\oplus}$) sign indicates the number of pairwise tests where the null hypotheses are rejected at \SI{1}{\percent} significance level. 
The plus ($^{+}$) sign indicates the number of pairwise tests where the null hypotheses are rejected at \SI{5}{\percent} significance level. 
%but not at \SI{1}{\percent}.
}

\begin{landscape}
\begin{table}[t]
    \caption{Evaluation scores for attributes on the main axes. \tablegend{}}
    % \tiny
    % \scriptsize
    \label{tab:main_scores}
    \setlength{\tabcolsep}{3pt}
    \renewcommand*{\arraystretch}{1.1}
    \centering
    \begin{tabularx}{\linewidth}{lp{3cm}*{15}{>{\raggedleft\arraybackslash}X}}
    \toprule
    Eng. Attr. &
    Trans. &
    \multicolumn{3}{c}{\uppercase{appr}} &
    \multicolumn{3}{c}{\uppercase{undr}} &
    \multicolumn{3}{c}{\uppercase{clar}} &
    \multicolumn{3}{c}{\uppercase{anto}} &
    \multicolumn{3}{c}{\uppercase{orth}} \\
    % \multicolumn{3}{c}{\uppercase{ncon}} &
    % \multicolumn{3}{c}{\uppercase{ibal}} \\
    \cmidrule(lr){3-5}
    \cmidrule(lr){6-8}
    \cmidrule(lr){9-11}
    \cmidrule(lr){12-14}
    \cmidrule(lr){15-17}
    && 
    Com & MY & SG &
    Com & MY & SG &
    Com & MY & SG &
    Com & MY & SG &
    Com & MY & SG \\
\midrule
annoying & membingitkan &  0.803 &  0.783 &  0.821 &  0.773 &  0.767 &  *\textbf{0.779} &  0.608 &  0.608 &  0.608 &  0.716 &  0.730 &  0.703 &  0.590 &  0.647 &  0.539 \\
           & menjengkelkan &  0.846 &  0.897 &  0.800 &  0.711 &  0.823 &            0.609 &  0.648 &  0.673 &  0.626 &  0.740 &  0.753 &  0.727 &  0.530 &  0.540 &  0.521 \\ \midrule
eventful & meriah &  0.673 &  0.677 &  0.670 &  0.929 &  0.960 &            0.900 &  0.540 &  0.585 &  0.500 &  0.586 &  0.603 &  0.570 &  0.416 &  0.467 &  0.370 \\\midrule
pleasant & menyenangkan &  0.840 &  0.857 &  0.824 &  0.910 &  0.900 &            0.918 &  0.526 &  0.557 &  0.498 &  0.624 &  0.647 &  0.603 &  0.613 &  0.633 &  0.594 \\\midrule
uneventful & tidak meriah &  0.713 &  0.737 &  0.691 &  0.902 &  0.920 &            0.885 &  0.579 &  0.630 &  0.532 &  0.668 &  0.677 &  0.661 &  0.695 &  0.687 &  0.703 \\\\
    \toprule 
    Eng. Attr. &
    Trans. &
    \multicolumn{3}{c}{\uppercase{ncon}} &
    \multicolumn{3}{c}{\uppercase{ibal}} \\
    \cmidrule(lr){3-5}
    \cmidrule(lr){6-8}
    % \cmidrule(lr){9-11}
    % \cmidrule(lr){12-14}
    % \cmidrule(lr){15-17}
    && 
    Com & MY & SG &
    Com & MY & SG \\
\midrule
annoying & membingitkan &            0.554 &  0.543 &  0.564 &             0.565 &  0.633 &            0.503 \\
           & menjengkelkan &  *\textbf{0.649} &  0.675 &  0.626 &  **\textbf{0.756} &  0.777 &  *\textbf{0.736} \\\midrule
eventful & meriah &            0.406 &  0.452 &  0.364 &             0.608 &  0.570 &            0.642 \\\midrule
pleasant & menyenangkan &            0.444 &  0.483 &  0.408 &             0.563 &  0.633 &            0.500 \\\midrule
uneventful & tidak meriah &            0.513 &  0.532 &  0.497 &             0.684 &  0.683 &            0.685 \\
\bottomrule
\end{tabularx}
\end{table}
\end{landscape}

==> unused/translations.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\newcolumntype{Z}{>{\raggedright\arraybackslash}X}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcolumntype{B}{>{\raggedright\arraybackslash}p{1cm}}
\begin{landscape}
\begin{table}[]
\centering
\caption{Translation process of the 8 PAQ attributes from English to Bahasa Melayu across all sub stages (1a to 1e) }
\label{tab:translations}
\begin{tabularx}{\linewidth}{lBZBZBZBZBZ}
\hline
\multicolumn{1}{l}{\multirow{2}{*}{Attribute}} & \multicolumn{2}{>{\centering\arraybackslash}p{4cm}}{Stage \textsc{1a}: Initial Translation} & \multicolumn{2}{>{\centering\arraybackslash}p{4cm}}{Stage \textsc{1b}: Focus Group Discussion}                                                                                         & \multicolumn{2}{>{\centering\arraybackslash}p{4cm}}{Stage \textsc{1c}: Pilot Evaluation}                                                     & \multicolumn{2}{>{\centering\arraybackslash}p{4cm}}{Stage \textsc{1d}: Preliminary  Translation}                                     & \multicolumn{2}{>{\centering\arraybackslash}p{4cm}}{Stage \textsc{1e}: Quantitative Evaluation (Final Provisional Translation)} \\
\multicolumn{1}{c}{}                         & Translations                  & Remarks            & Translations                          & Remarks                                                                                              & Translations                          & Remarks                                                    & Translations                         & Remarks                                              & Translations                      & Remarks                                 \\ \hline
eventful                                       & meriah                       &                    & meriah                                &                                                                                                      & meriah                                & unanimous                                                  & meriah                               & preferred across  stages 1a to 1c                    & meriah                            &                                         \\ \hline
vibrant                                        & bersemarak                   & preferred          & bersemarak                            & can be   accepted                                                                                    & bersemarak                            & difficult to   understand                                  & bersemarak                           & preferred in stages 1a and deemed   acceptable in 1b &                                   &                                         \\
                                               & rancak                       &                    & rancak                                & more layman                                                                                          & rancak                                & preferred by   most                                        & rancak                               & preferred in stages 1b and 1c                        & rancak                            & most understandable (inter & intra country)                    \\ \hline
pleasant                                       & menyenangkan                 &                    & menyenangkan                          &                                                                                                      & menyenangkan                          & unanimous;   accurate reverse translation by a participant & menyenangkan                         &                                                      & menyenangkan                      &                                         \\ \hline
calm                                           & tenang                       & preferred          & tenang                                &                                                                                                      & tenang                                & agreed by   most                                           & tenang                               &                                                      & tenang                            &                                         \\
                                               & tidak kecoh                  &                    & tidak kecoh                           & not   considered                                                                                     &                                       &                                                            &                                      &                                                      &                                   &                                         \\
                                               &                              &                    &                                       &                                                                                                      & menenangkan                           & means “calming”   thus not accepted                        & menenangkan                          &                                                      &                                   &                                         \\ \hline
uneventful                                     & tidak meriah                 & preferred          & tidak meriah                          & preferred in   parallel with “meriah”, as the English version is using “uneventful” and   “eventful” & tidak meriah                          &                                                            & tidak meriah                         &                                                      & tidak meriah                      &                                         \\
                                               & hambar dan   senyap          &                    & hambar dan   senyap                   & negative   connotation thus unsuitable as “uneventful” is neutral                                    &                                       &                                                            &                                      &                                                      &                                   &                                         \\ \hline
monotonous                                     & membosankan                  &                    & membosankan                           & agreed by   members                                                                                  & membosankan                           & agreed by   most                                           & membosankan                          &                                                      & membosankan                       &                                         \\
                                               &                              &                    & kurang   kepelbagaian dan membosankan & this will   translate both the “uneventful” and “unpleasant” aspects of the attribute                & kurang   kepelbagaian dan membosankan & double-barrelled                                           &                                      &                                                      &                                   &                                         \\
                                               &                              &                    &                                       &                                                                                                      & tidak berubah                         & means   “unchanging” only thus not suitable                &                                      &                                                      &                                   &                                         \\
                                               &                              &                    &                                       &                                                                                                      &                                       &                                                            & tidak berubah oleh itu   membosankan &                                                      &                                   &                                         \\ \hline
annoying                                       & membingitkan                 &                    & membingitkan                          & accurate but   may be uncommon                                                                       & membingitkan                          & understood,   unanimous                                    & membingitkan                         &                                                      & membingitkan                      &                                         \\
                                               &                              &                    & menjengkelkan                         & maybe   uncommon                                                                                     &                                       &                                                            & menjengkelkan                        &                                                      &                                   &                                         \\ \hline
chaotic                                        & kacau-bilau                  &                    & kacau-bilau                           &                                                                                                      & kacau-bilau                           & received   different opinions                              &                                      &                                                      &                                   &                                         \\
                                               &                              &                    &                                       &                                                                                                      & huru-hara                             & accepted to   describe atmosphere                          & huru-hara                            &                                                      & huru-hara                         &                                         \\
                                               &                              &                    &                                       &                                                                                                      & kelam-kabut                           & to describe a   place                                      & kelam-kabut                          &                                                      &                                   &                                         \\ \hline
\end{tabularx}
\end{table}
\end{landscape}
